Designing a Transactive Electric Vehicle Agent with Customer's Participation Preference

The proliferation of electric vehicles (EVs) and their inherent flexibility in charging timings make them an asset to improve grid performance. In contrast to direct control by a utility or autonomous price-based charging, the transactive control framework not only provides benefits to both grid and customers but also ensures customer autonomy. In this work, we design a transactive electric vehicle (TEV) agent that incorporates the EV owner's willingness to trade-off between savings and amenity in form of a slider, where the EV owner's amenity is characterized as vehicle readiness. Further, a privacy-preserving bidding formulation is proposed that also represents the customer's transactive preference. A transactive market mechanism is discussed that integrates the TEV Agents into the local retail market and reconciles with the current day-ahead and real-time market structure. It is demonstrated that the proposed slider is able to provide a preferred trade-off between savings and amenity to individual customers. At the same time, the market mechanism is shown to successfully reduce both peak prices and peak demand. A comparative investigation of V1G and V2G technologies with respect to the battery prices is also discussed.

==> old_changes.tex <==
The following citation was removed from "citation.bib"


@misc{taft2016architectural,
  title={Architectural basis for highly distributed transactive power grids: Frameworks, networks, and grid codes},
  author={Taft, JD},
  year={2016},
  publisher={June}
}



\cite{agent_EV_2017} utilize the transactive framework to deal with forecast errors. Having the EV agent behaving as shiftable loads or controlled charging rates depending of the real-time market.
\cite{agent_V2G_2017} EV agents have vehicle-to-grid (V2G) capabilities and respond to the real-time market. The EV and renewable energy sources (RES) uncertainties are considered. Thus, EV agent model is model as energy storage systems considering uncertainties. \cite{ZHENG2020115977} considers EV participating in day-ahead and real-time market with no V2G capabilities. The EV agents are aggregated and participate on the market with a centralize or decentralized mode. 


